Neural Time-Reversed Generalized Riccati Equation

Optimal control deals with optimization problems in which variables steer a dynamical system, and its outcome contributes to the objective function. Two classical approaches to solving these problems are Dynamic Programming and the Pontryagin Maximum Principle. In both approaches, Hamiltonian equations offer an interpretation of optimality through auxiliary variables known as costates. However, Hamiltonian equations are rarely used due to their reliance on forward-backward algorithms across the entire temporal domain. This paper introduces a novel neural-based approach to optimal control, with the aim of working forward-in-time. Neural networks are employed not only for implementing state dynamics but also for estimating costate variables. The parameters of the latter network are determined at each time step using a newly introduced local policy referred to as the time-reversed generalized Riccati equation. This policy is inspired by a result discussed in the Linear Quadratic (LQ) problem, which we conjecture stabilizes state dynamics. We support this conjecture by discussing experimental results from a range of optimal control case studies.

==> figs/fonts.tex <==
\input rotate % my versions of these files are in $CTAN/knuth/local/lib
\input picmac
\input epsf
\catcode`@=11 % borrow the private macros of PLAIN (with care)
\newdimen\clearance%(cellwidth-rulewidth-digitwidth)/2; set by \tenpoint

\let\del=\partial \newbox\ush \def\led{{\copy\ush}} % shadow and upper shadow
\newdimen\bitmapsize \bitmapsize=10pt

\font\ninerm=cmr9
\font\eightrm=cmr8
\font\sixrm=cmr6

\font\ninei=cmmi9  \skewchar\ninei='177
\font\eighti=cmmi8  \skewchar\eighti='177
\font\sixi=cmmi6  \skewchar\sixi='177

\font\tenbi=cmmib10  \skewchar\tenbi='177
\font\ninebi=cmmib9  \skewchar\ninebi='177

\font\ninesy=cmsy9  \skewchar\ninesy='60
\font\eightsy=cmsy8  \skewchar\eightsy='60
\font\sixsy=cmsy6  \skewchar\sixsy='60

\font\tenbsy=cmbsy10  \skewchar\tenbsy='60
\font\sevenbsy=cmbsy7  \skewchar\sevenbsy='60
\font\fivebsy=cmbsy5  \skewchar\fivebsy='60

\font\elevenex=cmex10 scaled\magstephalf
\font\nineex=cmex9
\font\eightex=cmex8
\font\sevenex=cmex7

\font\ninebf=cmbx9
\font\eightbf=cmbx8
\font\sixbf=cmbx6

\font\tenthinbf=cmb10
\font\ninethinbf=cmb10 at 9.25pt
\font\eightthinbf=cmb10 at 8.5pt

\font\twelvett=cmtt12  \hyphenchar\twelvett=-1  % inhibit hyphenation in tt
\font\tensltt=cmsltt10  \hyphenchar\tensltt=-1
\font\ninett=cmtt9  \hyphenchar\ninett=-1
\font\ninesltt=cmsltt10 at 9pt  \hyphenchar\ninesltt=-1
\font\eighttt=cmtt8  \hyphenchar\eighttt=-1
\font\seventt=cmtt8 scaled 875  \hyphenchar\seventt=-1

\font\ninesl=cmsl9
\font\eightsl=cmsl8

\font\nineit=cmti9
\font\eightit=cmti8

\font\eightss=cmssq8
\font\eightssi=cmssqi8
\font\sixss=cmssq8 scaled 800
\font\tenssbx=cmssbx10
\font\twelvess=cmss12
\font\titlefont=cmssbx10 scaled\magstep2

\font\tencsc=cmcsc10

\font\manfnt=manfnt % special symbols from the TeX project

\let\realtentt=\tentt
\def\tenpoint{\def\rm{\fam0\let\tentt=\realtentt\tenrm}%
  \clearance=4.175 pt
  \textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
  \textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\eightex \scriptscriptfont3=\sevenex
  \def\it{\fam\itfam\tenit}%
  \textfont\itfam=\tenit
  \def\sl{\fam\slfam\let\tentt=\tensltt\tensl}%
  \textfont\slfam=\tensl
  \def\bf{\fam\bffam\tenbf}%
  \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\tentt}%
  \let\sltt=\tensltt
  \textfont\ttfam=\tentt
  \scriptfont\ttfam=\seventt
  \def\oldstyle{\fam\@ne\teni}%
  \normalbaselineskip=12pt
  \def\bigfences{\textfont3=\elevenex}%
  \let\big=\tenbig
  \let\Big=\tenBig
  \let\bigg=\tenbigg
  \let\Bigg=\tenBigg
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
  \setbox0=\hbox{$\partial$}\setbox\ush=\hbox{\rotu0}%
  \bitmapsize=10pt
  \let\adbcfont=\eightrm
  \let\mc=\ninerm % for slightly smaller caps
  \let\boldit=\tenbi
  \let\ii=\tenii
  \def\MF{{\manfnt META}\-{\manfnt FONT}}%
  \normalbaselines\rm}

\def\ninepoint{\def\rm{\fam0\ninerm}%
  \clearance=3.9125 pt
  \textfont0=\ninerm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\ninei \scriptfont1=\sixi \scriptscriptfont1=\fivei
  \textfont2=\ninesy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\nineex \scriptfont3=\sevenex \scriptscriptfont3=\sevenex
  \def\it{\fam\itfam\nineit}%
  \textfont\itfam=\nineit
  \def\sl{\fam\slfam\let\ninett=\ninesltt\ninesl}%
  \textfont\slfam=\ninesl
  \def\bf{\fam\bffam\ninebf}%
  \textfont\bffam=\ninebf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\ninett}%
  \let\sltt=\error
  \textfont\ttfam=\ninett
  \def\oldstyle{\fam\@ne\ninei}%
  \normalbaselineskip=11pt
  \def\bigfences{\textfont3=\tenex}%
  \let\big=\ninebig
  \let\Big=\nineBig
  \let\bigg=\ninebigg
  \let\Bigg=\nineBigg
  \setbox\strutbox=\hbox{\vrule height8pt depth3pt width\z@}%
  \setbox0=\hbox{$\partial$}\setbox\ush=\hbox{\rotu0}%
  \bitmapsize=9pt
  \let\adbcfont=\sevenrm
  \let\mc=\eightrm % for slightly smaller caps
  \let\boldit=\ninebi
  \let\ii=\error
  \def\MF{{\manfnt hijk}\-{\manfnt lmnj}}%
  \normalbaselines\rm}
\let\normalninepoint=\ninepoint
\def\flexninepoint{\normalninepoint
  \advance\baselineskip 0pt plus .2pt minus .25pt}

\def\eightpoint{\def\rm{\fam0\eightrm}%
  \clearance=3.9125 pt
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti \scriptfont1=\sixi \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\eightex \scriptfont3=\sevenex \scriptscriptfont3=\sevenex
  \def\it{\fam\itfam\eightit}%
  \textfont\itfam=\eightit
  \def\sl{\fam\slfam\eightsl}%
  \textfont\slfam=\eightsl
  \def\bf{\fam\bffam\eightbf}%
  \textfont\bffam=\eightbf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\eighttt}%
  \let\sltt=\error
  \textfont\ttfam=\eighttt
  \def\oldstyle{\fam\@ne\eighti}%
  \normalbaselineskip=9pt
  \def\bigfences{\textfont3=\nineex}%
  \let\big=\eightbig
  \let\Big=\eightBig
  \let\bigg=\eightbigg
  \let\Bigg=\eightBigg
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width\z@}%
  \setbox0=\hbox{$\partial$}\setbox\ush=\hbox{\rotu0}%
  \bitmapsize=8pt
  \let\adbcfont=\sixrm
  \let\mc=\sevenrm % for slightly smaller caps
  \let\boldit=\error
  \let\ii=\eightii
  \def\MF{{\manfnt opqr}\-{\manfnt stuq}}%
  \normalbaselines\rm}

\def\tenbig#1{{\hbox{$\left#1\vbox to8.5pt{}\right.\n@space$}}}
\def\ninebig#1{{\hbox{$\textfont0=\tenrm\textfont2=\tensy
  \left#1\vbox to7.25pt{}\right.\n@space$}}}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}

\def\tenBig#1{{\hbox{$\bigfences
  \left#1\vbox to11.5pt{}\right.\n@space$}}}
\def\nineBig#1{{\hbox{$\bigfences
  \left#1\vbox to10.25pt{}\right.\n@space$}}}
\def\eightBig#1{{\hbox{$\bigfences
  \left#1\vbox to9.25pt{}\right.\n@space$}}}

\def\tenbigg#1{{\hbox{$\bigfences
  \left#1\vbox to14.5pt{}\right.\n@space$}}}
\def\ninebigg#1{{\hbox{$\bigfences
  \left#1\vbox to13pt{}\right.\n@space$}}}
\def\eightbigg#1{{\hbox{$\bigfences
  \left#1\vbox to11.5pt{}\right.\n@space$}}}

\def\tenBigg#1{{\hbox{$\bigfences
  \left#1\vbox to17.5pt{}\right.\n@space$}}}
\def\nineBigg#1{{\hbox{$\bigfences
  \left#1\vbox to15.75pt{}\right.\n@space$}}}
\def\eightBigg#1{{\hbox{$\bigfences
  \left#1\vbox to14pt{}\right.\n@space$}}}


%for Neurips

\font\timesfont=ptmr8r at 9pt
